Deeploy: Enabling Energy-Efficient Deployment of Small Language Models On Heterogeneous Microcontrollers

With the rise of Embodied Foundation Models (EFMs), most notably Small Language Models (SLMs), adapting Transformers for edge applications has become a very active field of research. However, achieving end-to-end deployment of SLMs on microcontroller (MCU)-class chips without high-bandwidth off-chip main memory access is still an open challenge. In this paper, we demonstrate high-efficiency end-to-end SLM deployment on a multicore RISC-V (RV32) MCU augmented with ML instruction extensions and a hardware neural processing unit (NPU). To automate the exploration of the constrained, multi-dimensional memory vs. computation tradeoffs involved in aggressive SLM deployment on heterogeneous (multicore+NPU) resources, we introduce Deeploy, a novel Deep Neural Network (DNN) compiler, which generates highly-optimized C code requiring minimal runtime support. We demonstrate that Deeploy generates end-to-end code for executing SLMs, fully exploiting the RV32 cores' instruction extensions and the NPU: We achieve leading-edge energy and throughput of \SI{490}{\micro\joule \per Token}, at \SI{340}{Token \per \second} for an SLM trained on the TinyStories dataset, running for the first time on an MCU-class device without external memory.

==> src/Acknowledgement.tex <==
\section*{Acknowledgment}


==> src/Rebuttal.tex <==
\vfill
\cleardoublepage
\glsresetall
\pagenumbering{gobble}

\section*{Responses to Reviewer Comments}

We thank the reviewers and editors for taking the substantial time to study and review our manuscript and providing constructive feedback. The insightful comments have allowed us to improve the paper further and revise points that needed to be explained more clearly. We appreciate the opportunity to revise and improve our manuscript, considering the comments we have received.

We have taken this revision as an opportunity to implement the reviewers' feedback and work on minor inconsistencies and typos in the paper. In the following, we provide detailed responses to each comment and elaborate on where and how we have modified the manuscript. 

We dedicate one Subsection to each reviewer's comments. We first copy the reviewer's feedback in \reviewer{darkgray} and address each comment individually below.
We highlight all relevant changes in \revA{red} for the reviewers' convenience. We will remove the highlighting in the camera-ready version.

\subsection{Comments to Reviewer 1}
\begin{quote}
\color{darkgray}

- The approach seem to rely heavily on the availability of specific hardware features like ML instruction extensions and NPUs, which may not be universally available on all microcontrollers. Moreover, It is unclear how the proposed methods would scale with larger models or more complex deployment environments.

- 'Deeploy' builds on existing kernel libraries and compilation techniques. It is not clear to me if the integration of these elements into a unified framework tailored for SLMs in edge environments is novel enough for this venue.

- The paper is comparing the performance of Deeploy with deployment frameworks on platforms like Apple or Samsung devices. These devices have different hardware architectures, capabilities, and power capabilities, which can make direct comparisons difficult and potentially misleading.

1) Why is "Quantization results" presented? From what I undertsand - you have used standard libraries.

2) If possible, I would like to see comparisons with existing compilers for the microcontroller used for Deeploy (not apple/samsung devices).
\end{quote}

First, we would like to thank the reviewer for their feedback, for raising their concerns about novelty and comparisons, and for pointing out ambiguities in our description of the results.

While we agree with the reviewer that \glspl{npu} and \gls{ml} \gls{isa} extensions are not universally available on all microcontrollers, there is a clear trend towards the integration of such units emerging \tinyml{}-capable \glspl{mcu}. Examples include \glspl{soc} integrating ARM's U55 and U85 accelerators, e.g. Alif Semiconductor's Ensemble E3\footnote{https://alifsemi.com}, but also other designs like STM's STM32N6 platform\footnote{https://blog.st.com/stm32n6/} Syntiant's NDP120\footnote{https://www.syntiant.com/hardware}, Greenwaves' GAP9\footnote{https://greenwaves-technologies.com/gap9\_processor/}, and many more. All of these platforms couple \gls{mcu} platforms (no OS, manual, DMA-based memory management, low amount of on-chip memory) with \glspl{npu} to accelerate \gls{dnn} inference. At the time of this writing, all these platforms focus on accelerating \glspl{cnn}; in our work, we propose an automated framework that can support not only \glspl{cnn} (as proved by our newer experiments, see the answer to your second question on MLPerf Tiny), but also the emerging paradigm of \glspl{slm}. To the best of our knowledge, ours is the first attempt to deploy such \glspl{slm} on a constrained \gls{npu}-augmented \gls{mcu}.

We would also like to stress that, while Deeploy is designed for generating highly optimized code for heterogeneous \gls{ml}-focused \glspl{soc}, neither \gls{ml} \gls{isa} extensions nor \glspl{npu} are required, thanks to the modular design of Deeploy's \platform{} abstraction.

We would further like to underline that besides integrating well-known compiler techniques in Deeploy, the novel static memory allocation and tiling algorithm presented in the paper is an essential contribution to this work. This static memory allocation and tiling algorithm guarantees strict upper bounds on memory utilization for complex dataflow networks, an important prerequisite for automatic deployment on tightly memory-constrained devices, a problem which has previously only been studied for simpler \gls{cnn} models. A further scientific contribution of this paper is deploying \glspl{slm} on this class of devices, which, to the best of our knowledge, has not been attempted before.

Concerning your first question, we present the quantization results, as, to the best of our knowledge, there is no literature about quantizing \glspl{slm} to achieve integer-only inference. We believe that even though quantization is not one of the core contributions of this paper, it is a necessary prerequisite for motivating the deployment of \glspl{slm} on extreme edge devices. Moreover, demonstrating that known quantization techniques apply to this class of models is a useful insight, especially considering that there is no established state-of-the-art for this class of networks on \gls{mcu}-class devices. However, to create space to address reviewers' feedback, and considering quantization is not a vital contribution of this work, we opted to remove the Section Quantization Results.

% \begin{quote}
%     \revA{To validate the proposed approach for deploying fully integerized \glspl{slm} on extreme edge devices, we present the average accuracy of the quantized model in a zero-shot setting, showing that standard quantization techniques are applicable to our \gls{slm} without loss of accuracy.}
% \end{quote}

Concerning your second remark, we agree that more comparisons with existing approaches would interest readers. However, to the best of our knowledge, there is no prior work in deploying \glspl{slm} on extreme edge devices. Similarly, we are not aware of work that has used prior tools to deploy \glspl{dnn} end-to-end on the Siracusa platform. 

Nevertheless, acknowledging the importance of the reviewer's request, we have carried out a comparison to evaluate the latency of code generated by different \tinyml{} compilers under comparable conditions. To this end, we have extended the open-source Dory tool to generate code for Siracusa, and compare it with Deeploy under equivalent conditions. While Siracusa offers an \gls{npu}, we exclude it for code generation in our comparison, as Dory does not feature support for it. We further disable the use of Siracusa's \gls{nms}.

Under these conditions, Dory and Deeploy generate code for equivalent platforms. We choose to compare all tools on the popular MLPerf tiny benchmark \cite{banbury_mlperf_2021}, which offers further comparison points for standardized \gls{cnn} workloads. Under these conditions, Deeploy performs equivalent to Dory, when using the same kernel libraries available open-source. To reflect this discussion, we have added a new Section termed "Comparison with tinyML Compiler":

\begin{quote}
\revA{While we designed Deeploy to deploy state-of-the-art and emerging \glspl{slm}, we also report results on more classical \gls{cnn} and \gls{ann} workloads, as defined in the MLPerf tiny benchmark \cite{banbury_mlperf_2021}. We compare Deeploy with the state-of-the-art open-source Dory tool \cite{burrello_dory_2021} using the same open-source \gls{cnn} kernels for PULP \glspl{mcu} \cite{garofalo_xpulpnn_2020} we used in this work. To ensure a fair, compiler-focused comparison, we do not use the \gls{nms} or the \glspl{npu} of Siracusa. In this mode, both compilers only deploy cluster kernels with equivalent memory constraints. As a third data point, we add measurements of Deeploy-generated code on Siracusa when using the \gls{nms} and \gls{npu}. Our results are shown in Table~\ref{tab:tinymlperf}. We find that Deeploy generates code with an equivalent latency of Dory up to 1\,\% of variation, underlining that even though Deeploy chooses a more general compilation approach than Dory, it does not incur any performance penalties.}
\end{quote}

\subsection {Comments to Reviewer 2}
\begin{quote}
\color{darkgray}
- The experimental results are promising considering resource constraint environment and running on hardware instead of simulation.

1) The main results like average energy cost of 490 uJ per token and throughout of 340 token/s are not mentioned in the results section. Energy efficiency can be deduced from 27 mJ/token / 55x in Section VI-F but they should be presented in a table or text in Section VI other than introduction and conclusion.

2) The motivation to profile the performance of encoder layer of Transformer models is missing as the deployed Llama model is a decoder-based language model.
\end{quote}

We thank the reviewer for their comments and agree that the energy efficiency and throughput figures should be clarified in the results section, and the motivation for encoder layer measurements can be improved.

Concerning your first remark, Table II in the manuscript lists the cumulative latency and energy cost of executing the network over 256 steps, which we take as the baseline for our energy and throughput calculations. Consequently, the average energy cost and throughput are calculated by dividing the measurements in autoregressive inference mode by 256, the number of inference steps for the measurement. We have added a paragraph in the results section to reflect this discussion:

\begin{quote}
Table~II displays the cumulative runtime and energy for executing a 256-step inference in parallel mode and in autoregressive mode, where $KV$ caching is used. The autoregressive mode outperforms the parallel mode, achieving a 23\,$\times$ speedup and a 26\,$\times$ improvement in energy efficiency. These improvements directly result from avoiding the costly recomputation of $KV$ matrices. \revA{Averaging the autoregressive inference mode's cumulative latency and energy in autoregressive inference mode over 256 steps, we achieve an average throughput of \SI{340}{token \per \second} at an average energy cost of \SI{490}{\micro\joule \per token}.}
\end{quote}

Concerning your second remark, we agree that the motivation for Figure~\ref{fig:parallel} and the encoder layer results are unclear. While our key results are calculated from measurements of the autoregressive inference mode of decoder-only models, Deeploy also supports the parallel inference mode, as well as mixed decoder- and encoder-based models. Generally, the parallel inference mode in decoder-only models is equivalent to the encoder layers of standard transformer models. In this sense, the numbers presented in the paper are applicable for both the parallel inference mode and encoder layers, given equal hyperparameters. To clarify this fact and add motivation, we modified a paragraph in the manuscript:

\begin{quote}
\revA{The parallel inference mode's performance for the \glspl{slm} studied in this work follows the trend of the benchmark shown in Figure~\ref{fig:parallel}. While we benchmark the end-to-end performance of decoder-only models in this work, the results in Figure~\ref{fig:parallel} also apply to encoder-based transformer models, as the parallel inference mode is equivalent to encoder layer execution in such networks.}
\end{quote}

\subsection{Comments to Reviewer 3}

\begin{quote}
\color{darkgray}

1) The authors use a front end to generate the IR. In doing so how do the authors perform layer fusion and splitting based on the NPU or platform that is used. This is needed for the design space exploration (DSE).

2) Buffer allocation in the context of heterogeneous platforms is complicated. For example, depending on the resource constraints and if streaming is enabled, the buffers will be reused all the time with spills. If the CPU is the one doing the FP32 ops then does the compiler here in question provide knobs to help perform these allocations for the user to perform DSE the way they want to.

3) The comparison to R[54] is done by deploying the same model on the same platform? It is not clear how this has been done.

4) There needs to be more results showing how the buffer utilization happens, code size, time for compilation, and scalability to evaluate the proposed compiler.

\end{quote}

We thank the reviewer for their feedback. We agree that additional results on code size, compilation time, and scalability could improve the manuscript. We also agree that our explanations of buffer allocation and the proposed comparisons could benefit from clarification.

We want to clarify that our paper does not directly address the problem of design space exploration (DSE). At the same time, DSE is an important topic in heterogeneous accelerator \glspl{soc}; our work is focused on reliable code generation for software-managed scratchpad-based architectures rather than exploring different mapping and scheduling trade-offs.

Concerning your first question: The layer fusion and splitting rules in the Frontend are entirely configurable by the user to address the specific lowering requirements of the targeted hardware platform; To implement this flexibility, Deeploy uses platform-specific and adaptable lowering passes, which match source subgraph patterns and replace them by target subgraphs. This replacement may use information stored within the matched source pattern to compute the replacement pattern. Based on heuristics that are not currently captured in Depeloy, future work might expand this flexible system to incorporate information from higher-level tools like CoSA \cite{huang_cosa_2021} or others to enable increasingly fine-grained Design Space Exploration. We added a paragraph in Section Frontend to capture this discussion:
\begin{quote}
    
Deeploy implements a configurable lowering pass system based on pattern matching of \gls{onnx} graphs to enable efficient and customizable graph-lowering strategies. \revA{Each lowering pass consists of a user-defined replacement function and a \textit{source pattern}, which describes the sub-graph that should be replaced. Each lowering pass uses the matched sub-graph with a pre-defined replacement function to generate a \textit{target pattern}, which replaces the \textit{source pattern}.}

\end{quote}

Concerning your second remark: The current implementation of the buffer allocation algorithm in Deeploy is coupled to the tiling implementation; Deeploy first computes a static execution schedule of all operators in the network and uses this schedule to calculate the lifetime of all required tensor memory buffers. The \gls{cp} based tiling algorithm uses this lifetime information to allocate a fixed memory address for all required memory locations in all memory hierarchy levels they need. Implementing the solution to this algorithm guarantees that no unscheduled spills between memory hierarchy levels are necessary, and the compiler generates all required memory transfers. The user may further define heuristics to steer the computation of tiling solutions with per-engine granularity, which impacts the frequency and configuration of such memory transfers.

We added two additional paragraphs in the manuscript to reflect this discussion:

\begin{quote}
The \middleware{} performs all tiling and static memory allocation computations\revA{, guaranteeing that the computed program schedule may execute without unscheduled runtime memory spills}.
\end{quote}

\begin{quote}
    Using this system, the first processing step in the Frontend is transforming the input graph into a custom, platform-specific ONNX dialect using lowering passes provided by the Deployment Platform. \revA{The user further defines operator mappings between custom operators and the engines available in the target platform to control the code generation on the level of individual operators.} 
\end{quote}

Concerning your third remark: The comparison with \cite{liu_mobilellm_2024} is made between the estimated energy consumption of a larger \gls{slm} on an iPhone 13 application-class processor by the authors of \cite{liu_mobilellm_2024}, and the deployment of the proposed \gls{slm} on Siracusa. The comparison shows that our deployment results on Siracusa are comparable in terms of throughput \& energy efficiency when normalizing for the number of operations of both models.

We agree this comparison is not perfect; however, to the best of our knowledge, no implementation of an \gls{slm} on a microcontroller-class device has been reported in literature. We believe that offering at least this data point to compare our implementation with is interesting for readers to gauge the merit of our work.

Nonetheless, we agree that we should clarify the exact comparison setup, and therefore, we amended the result section as follows:

\begin{quote}
Compared to this estimate \revA{on the iPhone 13's A15 processor, the implementation of the proposed \gls{slm} on the Siracusa microcontroller} uses 26\,$\times$ less energy per token while achieving 5\,$\times$ more throughput, for a total 130\,$\times$ higher energy efficiency. When normalizing throughput with the number of operations per token of their network, we find that they achieve an equivalent of 4800 TinyStories Llama tokens per second. Under this estimate, our end-to-end energy efficiency on Siracusa implemented in an older \SI{16}{\nano\meter} TSMC technology node is 1.7$\,\times$ higher.
\end{quote}

Concerning your fourth remark, we agree that compiler performance metrics are interesting to the ESWEEK CASES audience. Therefore, we add an experiment to determine the scaling of code size, compilation time, and I/O memory buffer utilization for \glspl{slm}. 

In detail, we analyze the 128th inference step of the autoregressive inference. We vary the number of decoder layers between 1 and 8 and measure the total number of deployed operators, the processing time of Deeploy, and the .text and .data sections of the generated binary. We further break down the contents of the .data section into weights \& parameters stored in L2, i.e., not in the \gls{nms}, and I/O buffers. We also report the data stored in the \gls{nms}. The results are shown in Table~\ref{tab:compiler_metrics}. 

We added Section~\ref{sec:compilermetrics} to reflect this discussion, which reads as follows: 

\begin{quote}
\revA{To study the scalability of our code generation approach, we break down the \gls{slm} network, measuring compiler metrics for varying network depth. For each configuration, we profile code size, constant data size, and input- and output buffer size for a single inference step in \scenarioFour{}, namely the 128th autoregressive inference step. Our results are shown in Table~\ref{tab:compiler_metrics}.}

\revA{We notice that while code size grows proportionally to the number of operators in the workload, the total size of the binary is dominated by weight storage in the \gls{nms}. }

\revA{We further find that while compilation time grows superlinearly with the number of operators in the network, the maximum compilation time of \SI{28}{\second} does not pose a bottleneck for practical purposes.}

\end{quote}


\vspace{\fill}
\eject

\cleardoublepage

==> tab/averageAccuracy.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of Average Accuracy}
% \caption{Comparative Analysis of Zero-Shot Task Performance. The accuracy is averaged across various tasks, including Helloswag, OpenBookQA, WinoGrande, ARC-Easy, ARC-Challenge, BoolQ, and PIQA using the Language Model Evaluation Harness developed by EleutherAI.}
\label{tab:avg_accuracy}
\begin{tabularx}{\linewidth}{Xcc}
\hline
\textbf{Model}                    & \textbf{Type} & \textbf{Avg Accuracy (\%)} \\ \hline
TinyLlama-5M           & BF16         & 31.59 $\pm$ 1.09 \\
\textbf{TinyLlama-5M}          & \textbf{INT8 PTQ} & \textbf{32.15 $\pm$ 1.11} \\ \hline
TinyStories-GPT2-3M      & FP32         & 32.29 $\pm$ 1.11 \\
TinyStories-3M           & FP32         & 32.61 $\pm$ 1.10 \\
TinyStories-8M           & FP32         & 36.79 $\pm$ 1.13 \\
TinyStories-33M          & FP32         & 35.63 $\pm$ 1.13 \\
GPT-Neo 125M             & FP32         & 40.39 $\pm$ 1.15 \\
MobileLLM 125M           & FP32         & 47.00 \\
TinyLlama-1.1B-Chat-v0.4 & FP32         & 49.41 $\pm$ 1.23 \\ \hline
\end{tabularx}
\end{table}

==> tab/averageNormalizedAccuracy.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{Comparison of Average Normalized Accuracy of Different Models}}
\label{tab:avg_normalized_accuracy}
\begin{tabularx}{\linewidth}{Xcc}
\hline
\textbf{Model}           & \textbf{Type} & \textbf{Avg Normalized Accuracy (\%)} \\ \hline
TinyLlama-5M             & BF16         & 36.91 $\pm$ 1.20 \\
\textbf{TinyLlama-5M}    & \textbf{INT8 PTQ} & \textbf{37.41 $\pm$ 1.21} \\ \hline
TinyStories-GPT2-3M      & FP32         & 33.59 $\pm$ 1.18 \\
TinyStories-3M           & FP32         & 37.14 $\pm$ 1.18 \\
TinyStories-8M           & FP32         & 37.76 $\pm$ 1.19 \\
TinyStories-33M          & FP32         & 38.30 $\pm$ 1.21 \\
GPT-Neo 125M             & FP32         & 42.09 $\pm$ 1.23 \\
TinyLlama-1.1B-Chat-v0.4 & FP32         & 52.83 $\pm$ 1.28 \\ \hline
\end{tabularx}
\end{table}
